Prototype Schwarzschild-Couder Telescope for the Cherenkov Telescope Array: Commissioning the Optical System

A prototype Schwarzschild-Couder Telescope (pSCT) has been constructed at the Fred Lawrence Whipple Observatory as a candidate for the medium-sized telescopes of the Cherenkov Telescope Array Observatory (CTAO). CTAO is currently entering early construction phase of the project and once completed it will vastly improve very high energy gamma-ray detection component in multi-wavelength and multi-messenger observations due to significantly improved sensitivity, angular resolution and field of view comparing to the current generation of the ground-based gamma-ray observatories H.E.S.S., MAGIC and VERITAS. The pSCT uses a dual aspheric mirror design with a $9.7$ m primary mirror and $5.4$ m secondary mirror, both of which are segmented. The Schwarzschild-Couder (SC) optical system (OS) selected for the prototype telescope achieves wide field of view of $8$ degrees and simultaneously reduces the focal plane plate scale allowing an unprecedented compact ($0.78$m diameter) implementation of the high-resolution camera ($6$mm/ $0.067$deg per imaging pixel with $11,328$ pixels) based on the silicon photo-multipliers (SiPMs). The OS of the telescope is designed to eliminate spherical and comatic aberrations and minimize astigmatism to radically improve off-axis imaging and consequently angular resolution across all the field of view with respect to the conventional single-mirror telescopes. Fast and high imaging resolution OS of the pSCT comes with the challenging submillimeter-precision custom alignment system, which was successfully demonstrated with an on-axis point spread function (PSF) of $2.9$ arcmin prior to the first-light detection of the Crab Nebula in 2020. Ongoing and future commissioning activities are reported.

==> optical_alignment_overview.tex <==
The optical PSF is most sensitive to the tip/tilt rotation of the M1 and M2 panels and also the translations of the M2 panels. These degrees of freedom are constrained using de-focused images of stars.
This section provides a brief summary of the optical alignment procedure when the inner ring of S1 panels of M2 is assumed to be aligned (see next section). For more detailed information on this alignment procedure and earlier results, see \cite{Adams2020, Adams2020a}.

The de-focused image of a star is created by the reflection from a pair of M1 and M2 panels in which each panel is purposely misaligned to form patterns of rings of individual pairs so that the 80 images created by all possible pairs in the OS are identifiable.  

Images of a star produced by pairs of panels P1-S1, P2-S1, and P2-S2 are arranged into three concentric ring configurations, which are shown in Figure~\ref{fig:optical_alignment_overview}: the aligned panels in the focused configuration are shown in Figure~\ref{fig:optical_alignment_overview} (A), while two different states of the de-focused configuration are shown in Figures~\ref{fig:optical_alignment_overview} (B) and (C).
These de-focused configurations facilitate easy identification of images produced by each combination of primary and secondary panels and enables simultaneous and efficient alignment of each image into the predetermined pattern, which must be produced by a star. In addition, the characteristics of individual images (major and minor axes and elongation) are used to guide the relative global positioning of M1, M2 and FP.

To relate the motion of the images on the FP to the adjustments of the actuators of Stewart platforms, the response matrices for each panel are simultaneously measured at the 3-ring configuration (Figure~\ref{fig:optical_alignment_overview} (C)) by rotating (tip and tilt) each mirror panel and observing the motion of the corresponding focal-plane image.

Based on the response matrices, the displacement between predetermined pattern of pairs of images of the star with respect to the focal point can be used to guide the precise tip/tilt rotation of each panel in order to achieve the focus of the OS. This procedure using measured response matrices constitutes the zeroth-order alignment of the mirror panels, which is not yet ideal because the response matrices are measured at the 3-ring configurations instead of at the focused configuration where linear approximation may be insufficient. To further improve alignment, the development of the 1st-order alignment correction at the focal point is currently in progress. 


% \cite{Adams2020} % Qi proceeding, SPIE
% \cite{Adams2020a} % Ruo proceeding, SPIE
% \cite{Rousselle13} %spie
% \cite{Nieto15} % icrc15
% \cite{Rousselle2015} % spie
% \cite{Nieto:2017cyj} % icrc17
